Barely Random Algorithms and Collective Metrical Task Systems

We consider metrical task systems on general metric spaces with $n$ points, and show that any fully randomized algorithm can be turned into a randomized algorithm that uses only $2\log n$ random bits, and achieves the same competitive ratio up to a factor $2$. This provides the first order-optimal barely random algorithms for metrical task systems, i.e., which use a number of random bits that does not depend on the number of requests addressed to the system. We discuss implications on various aspects of online decision-making such as: distributed systems, advice complexity, and transaction costs, suggesting broad applicability. We put forward an equivalent view that we call collective metrical task systems where $k$ agents in a metrical task system team up, and suffer the average cost paid by each agent. Our results imply that such a team can be $O(\log^2 n)$-competitive as soon as $k\geq n^2$. In comparison, a single agent is always $\Omega(n)$-competitive.

==> packages-arxiv.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
%\usepackage[dvipsnames]{xcolor}         % colors

%%%%% NEW PACKAGES 
\usepackage{amsthm}
\usepackage{amsmath,amssymb}% added for align
\usepackage{comment}        % added for comment
\usepackage{enumitem}  %for "the following statements are equivalent"
\usepackage{parskip}
\usepackage{cleveref} %%NNNEWW

\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{lemma}[theorem]{Lemma}

\providecommand{\keywords}[1]{\textbf{Keywords: } #1}
%\newtheorem{definition}[theorem]{Definition}

%\newtheorem{corollary}{Corollary}[theorem]
%\newtheorem{assumption}{Assumption}[section]
%\newtheorem{claim}{Claim}[section]
